Offline Reinforcement Learning as One Big Sequence Modeling Problem

Reinforcement learning (RL) is typically concerned with estimating stationary policies or single-step models, leveraging the Markov property to factorize problems in time. However, we can also view RL as a generic sequence modeling problem, with the goal being to produce a sequence of actions that leads to a sequence of high rewards. Viewed in this way, it is tempting to consider whether high-capacity sequence prediction models that work well in other domains, such as natural-language processing, can also provide effective solutions to the RL problem. To this end, we explore how RL can be tackled with the tools of sequence modeling, using a Transformer architecture to model distributions over trajectories and repurposing beam search as a planning algorithm. Framing RL as sequence modeling problem simplifies a range of design decisions, allowing us to dispense with many of the components common in offline RL algorithms. We demonstrate the flexibility of this approach across long-horizon dynamics prediction, imitation learning, goal-conditioned RL, and offline RL. Further, we show that this approach can be combined with existing model-free algorithms to yield a state-of-the-art planner in sparse-reward, long-horizon tasks.

==> figures/imitation.tex <==
\begin{wrapfigure}[18]{r}{0.35\linewidth}
    \vspace{-0.25cm}
    \centering 
    \includegraphics[width=0.98\linewidth]{images/imitation.pdf}
    \caption{
    \textbf{(Imitation learning)}
    We find that TTO, despite being built on the tools of natural language processing instead of behvior cloning, is a capable imitative method.
    Performance of the behavior cloning (BC) baseline is taken from \citep{kumar2020conservative}.
    }
    \label{fig:imitation}
\end{wrapfigure}

